The Life and Death of Unwanted Bits: Towards Proactive Waste Data Management in Digital Ecosystems

Our everyday data processing activities create massive amounts of data. Like physical waste and trash, unwanted and unused data also pollutes the digital environment by degrading the performance and capacity of storage systems and requiring costly disposal. In this paper, we propose using the lessons from real life waste management in handling waste data. We show the impact of waste data on the performance and operational costs of our computing systems. To allow better waste data management, we define a waste hierarchy for digital objects and provide insights into how to identify and categorize waste data. Finally, we introduce novel ways of reusing, reducing, and recycling data and software to minimize the impact of data wastage

==> model.tex <==
\section{Model}
\label{sec:model}

This is the model section.

==> solution.tex <==
\section{Principles of Waste Data Management}
\label{sec:solution}
\label{sec:principles}
We propose several techniques for managing waste data.


\noindent\textbf{Digital Landfills.~} A digital landfill is the equivalent of real-life landfills, where unwanted data can be disposed of without additional cost associated with deletion. For this, we propose using a semi-volatile storage device. Such a storage device would store data, but gradually unwanted data objects will fade and the storage space can be reclaimed. This type of device can be implemented on a volatile storage medium using a least-recently-used (LRU) scheme, where data not recently used will be allowed to fade, while more frequently used data will be refreshed. \\

\noindent\textbf{Waste penalties for applications.~} A \textit{waste penalty} can be imposed on applications that create large amounts of waste data. For example, the operating system can penalize an application that creates a lot of temporary files by reducing its I/O bandwidth or schedule it to receive fewer CPU cycles. This gives applications incentives to act responsibly in creating waste data. This concept is equivalent to the \textit{Pay-as-You-Throw} scheme used in real-life waste management.\\


\noindent\textbf{Micro-modular software.~} A big problem with recycling old or unwanted software is that software libraries are not usually written to allow extraction of small amounts of code. Shared dynamic link libraries (DLL) do allow code sharing among multiple applications. However, DLLs do not allow removal of unused routines to retain only the routines that are used. When recycling a library, it is therefore not possible to extract usable routines from it. To allow recycling old code, we propose breaking up software code libraries in to micro-modules in the level of individual routines or algorithms, which can be extracted from the library when recycling old code.\\
